A Detailed Description of the CamSpec Likelihood Pipeline and a Reanalysis of the Planck High Frequency Maps

This paper presents a detailed description of the CamSpec likelihood which has been used to analyse Planck temperature and polarization maps of the cosmic microwave background since the first Planck data release. We have created a number of likelihoods using a range of Galactic sky masks and different methods of temperature foreground cleaning. Our most powerful likelihood uses 80 percent of the sky in temperature and polarization. Our results show that the six-parameter LCDM cosmology provides an excellent fit to the Planck data. There is no evidence for statistically significant internal tensions in the Planck TT, TE and EE spectra computed for different frequency combinations. We present evidence that the tendencies for the Planck temperature power spectra to favour a lensing amplitude A_L>1 and positive spatial curvature are caused by statistical fluctuations in the temperature power spectra. Using our statistically most powerful likelihood, we find that the A_L parameter differs from unity at no more than the 2.2 sigma level. We find no evidence for anomalous shifts in cosmological parameters with multipole range. In fact, we show that the combined TTTEEE likelihood over the restricted multipole range 2-800 gives cosmological parameters for the base LCDM cosmology that are very close to those derived from the full multipole range 2-2500. We present revised constraints on a few extensions of the base LCDM cosmology, focussing on the sum of neutrino masses, number of relativistic species and the tensor-scalar ratio. The results presented here show that the Planck data are remarkably consistent between detector-sets, frequencies and sky area. We find no evidence in our analysis that cosmological parameters determined from the CamSpec likelihood are affected to any significant degree by systematic errors in the Planck data (abridged).

==> notes.tex <==
1. Introduction:  Added summary paragraphs as requested.
2. Page 4:   The residual means come from Galactic foreground -- tex modified.
3. Page 5:   text modified. Exact match of beams to sky area is not critical for isotropised 
             power spectra. For example, one can safely use 75pc sky beam transfer
             functions available on the PLA to model spectra computed on 60pc 
             of sky.  The differences are small compared to the errors on the  
             spectra.
4. Page 5:   Non-gaussianity of foregrounds addressed in text.
5. Page 5:   We have explained why the Gaussian approximation underestimates the amplitude of the
             CMB-dust correlations in a footnote. However, am a bit puzzled by the comment in the
             report because the ensemble average is not relevant here.
6. Section 3.  The referee is correct that weighting appropriately can minimise the variance in the
              PCL estimates. As discussed in Efstathiou 2004 (E04), the optimal choice is to use equal 
              weights per pixel in the signal dominated regime and inverse noise-variance weighting
              in the noise dominated regime. It is even possible, as discussed in E04,  to construct hybrid estimators to 
              deal with spectra in multipole ranges that are neither signal nor noise dominated. For
              Planck, we decided to keep the covariance matrix calculations simple, so we used the
              apodised weight functions (equal weight per pixel over most of the sky) for all spectra.
              We have added a footnote explaining this and referencing E04. 
7.            Units added in text just below Table 2.
8.            Fig. 5.1  Colour of U noise spectra changed to green.
9.            Have modified the text on pages 12 and 13 on noise estimation. The empirical noise estimates
              for 100 GHz are unsatisfactory; both HRD and OED noise estimates match the noise levels at high
              multipoles but have different shapes at low multipoles. The ffp10 simulations do not accurately 
              model sources of non-white noise. One of our PhD students is currently investigating whether 
              the latest end-to-end simulations of the HFI and NPIPE processing can be used to construct more reliable 
              noise covariance matrices following techniques similar to those described in de Belsunce etal 2021. 
10.           p16  added reference to Hivon etal  (ref 36) for the \ell^m model in Eq. 6.6.
11.           One should worry about errors in the polarization angles. There may indeed be systematics in the EE
              spectra associated with polarization angles and this may be one of the reasons for the mismatch of 
              EE and TE polarization efficiencies plotted in Fig. 6.2.  We have added additional comments on pages 14 
              and 15. The (dust subtracted) TB and EB spectra are consistent with the ground based polarization 
              angle errors and also with a small offset in the orientation of the focal plane (have added a reference to this).               However, the effective polarization efficiencies vary by several times the error quoted by Rosset etal. 
              and so the assumption that polarization efficiencies dominate the EE systematic error budget is well motivated.
12.           spelling of `publicly' corrected
13.           the source of the CO mask used in this paper, and in the Planck data releases is given on page 8.
14.           B-mode foregrounds. We think that it is going beyond the scope of this paper to say more about the 
              most effective strategy for future B-mode experiments. We would need to do extensive simulations. 
              For Litebird, the choice has already been made to sample a very wide frequency range from 40-402 GHz.
              Our hunch is that the polarized synchrotron spectral index will vary strongly over the sky and that
              foreground separation at low multipoles will be much more accurate at the dust dominated higher 
              frequencies -- but we will see if and when Litebird returns data.
15.           Table 8. I didn't see a problem here. alpha_B is a bit higher than alpha_E for 217 GHz and a bit lower
              for 143 and 100 GHz. The key point is that the numbers are very similar, and because the minima
              are very broad (explained in Eq. 7.12)  it wouldn't make any significant difference had we used alpha_B
              or alpha_E.
16.           The spectral indices epsilon^EE, epsilon^BB are expected to differ from the spectral index in 
              temperature because Galactic polarized emission is related to the   power spectrum of interstellar 
              magnetic field. Have added a reference to Ghosh etal 2017, on page 34, in which this is explained in
              detail.
17.           Actually there were typos in Table 10. All of the dust priors were listed with sigma = 0.02, whereas
              they should be sigma = 0.2. These errors have been corrected. Via mask differencing we can determine
              the shapes of the dust templates very accurately. The absolute amplitudes are more problematic, however,
              because in addition to the fluctuations seen in Table 7, we need to correct for the dust amplitudes 
              at high Galactic latitudes, which requires an analysis to separate dust from extragalactic foreground. 
              To avoid overcomplicating matters we used a generous prior of 20\% error on the amplitudes. 
              If we look at the errors on the dust amplitudes for the 12.1 likelihood we find: 
                                       
                                       mean     ssdev
                          100x100     1.15      0.19
                          143x143     0.79      0.15
                          217x217     0.87      0.09
                          143x217     0.97      0.16

            so the choice of 20\% errors is not too bad -- only the
            error on the 217x217 dust amplitude is tighter than its
            prior (which we could have anticipated from Table 7). 

 18.  Combining low ell and high ell likelihoods, including
            covariances is discussed in Efstathiou, 2004, MNRAS, 349,
            603.  In the case of the Planck likelihoods, the low ell
            likelihood is a maximum likelihood solution covering a
            large area of sky and so the C_ell covariance matrix is
            almost diagonal at ell=29. There will be a small
            inconsistency matching to the pseudo C_ell estimates at
            ell>29, (which are correlated over a multipole range set
            by the size of the mask) but cosmic variance is so huge at
            these multipoles that any mismatch would have an
            imperceptible effect on the combined low ell-high ell
            likelihood. Since the first Planck data release we decided
            to treat the the low-ell and high-ell likelihoods as
            independent and we are very sure that this is a very good
            approximation.  

19.         Fixed text in Section 10.2 and added a reference to de Belsunce etal (2021) (investigating
            low-ell likelihood approximations).  

20.         Error bars on
            the band-averaged CamSpec points are plotted in
            Fig. 10.3. We have had to change the scale of the ordinate
            to fit these error bars on the plot.  
21.          A K-S test is
            inappropriate here. The key point in Fig. 11.1, 11.2, 11.3
            etc and 13.11 in particular, is to test the consistency of
            the power spectra for different frequency combinations
            point-by-point.  Fig. 13.11 is the most stringent test and
            shows fantastic consistency between the band-averaged
            points and is a technically demanding quantitative test
            since the errors account for noise and cosmic variance
            associated with the slight differences in the masks. 

 22.        At the start of the paper, we stated that cosmological
            parameters were defined as in PCP18 to avoid having to
            define theta_*, r_{drag}, A_s, sigma_8, S_8, etc, which
            would have required a lot of repetition. Nevertheless, we
            have said this again in the caption to Fig. 13.2. (It
            doesn't make a lot of sense to define S_8 in terms of
            sigma_8 and Omega_m, if we haven't defined sigma_8. S_8 is
            defined explicitly just before Eq. 13.4.)  

23.         Have added text to get the point across more clearly. The default
            foreground model used since PCP13 was never intended to be
            used for multipole cuts. For example, Galactic dust is
            dominant only at low multipoles -- so if you cut at
            l>1000, dust becomes degenerate with CIB and point
            sources. Any error in the shapes of these templates (and
            there is considerable error in the shape of the CIB
            templates) will couple to n_s and other parameters. This
            is the main cause of the differences between Addison etal
            and the results of this section. Also, the polarization
            results presented here argue against parameter shifts of
            physical (rather than statistical) being the cause of the
            differences between Planck and WMAP.  
25.          We have been through the paper and checked the formatting.  
26.         The  analysis of arXiv:2010.01139 is flawed at many levels. The
            likelihoods used for low ell analysis have no theoretical
            basis and given the noise levels and residual systematics
            in Planck polarization, the claim of r< 0.069 is totally
            implausible. This limit conflicts with the 95\% limit of
            $r<0.41$ from low multipole analysis of the SROLL1 maps
            quoted in PPL18. One of us looked at the constraints from
            the SROLL1 maps and found a 1\sigma upper limit of $r< 0.33$
            which we didn't think worth publishing. To argue that the
            joint Planck+BICEP/Keck constraint improves to r< 0.044
            does a disservice to the careful work of the BICEP/Keck
            team. We have added a reference to this paper in a footnote 
            on page 81, with appropriate comments. 


==> referee_reply.tex <==

We are prepared to make minor revisions to the paper, expressing
points more clearly and adding clarifications. However, we are not
prepared to make major revisions to this paper, for the reasons
described below.

We don't envy the referee for having to read such a long
paper. However, the report was very antagonistic and unconstructive.
We were actually quite shocked at the number of errors and
misconceptions in the report. There was also no recognition that one
of the main aims of the paper was to push the Planck data to create a
more powerful likelihood. As we say in the paper, if `tensions' such
as outliers, parameter shifts, A_L, Omega_k etc are statistical
fluctuations, even a modest improvement in the likelihood will cause
these tensions, statistically, to become less significant.  This is
exactly what we find. This is an important result.

Every comment from the referee was negative (even when dealing with
well trodden points described in the Planck collaboration papers). As
such, there is far too much that divides us to reach a compromise.
There is simply no appreciation by the referee of the amount of
thought, work and testing that has gone into this paper.

Planck was a near billion euro project and has redefined
cosmology. Although the paper is long, we think that the length and
technical detail is justified because of the significance of the
Planck project. It will stay significant for many years. This paper
presents a coherent account of the CamSpec likelihood in a single
source. It is not possible to get an equivalent account at this level
of detail from the Planck likelihood papers, either for CamSpec or
Plik.

To be clear about our position, we will go through the points on pages
6-20 in some detail.


2.1 The beam window functions are computed on nearly the same sky
areas as the spectra used for most of the likelihoods. We know from
quickpol that changes of even 20\% of sky area cause very small
changes to the effective beams. In Eq. (2.6b) one wants to be able to
apply beam corrections to the mask deconvolved spectra (and to coadd
spectra) otherwise you have to do the deconvolution every time you
want to evaluate the likelihood. The approximation of equation (2.6b)
is justified because $W_\ell$ is a slowly varying function of $\ell$
as stated in the text.  It is strange to be asked to justify the use
of ell-by-ell spectra!  Binning loses information, and it is actually
important for testing models such as axion monodromy. We did not have
to bin in multipole because our combined TTTEEE likelihood is much
more compact than the Plik likelihood.  This is surely a positive.


2.2 The point source mask adds a bit of extra variance, but it is a
small contribution to cosmic variance. This is discussed in the 2015
Planck Likelihood paper. As a consequence neither we nor the Plik team
correct the covariance matrices for point source leakage. GE
introduced the heuristic $\psi_\ell$ corrections in the 2013 Planck
papers. It locally corrects the white noise level and gives a good
match to the scatter of the spectra in the noise dominated regime at
high multipoles. It is however, heuristic. The Planck simulations are
not good enough to test this approximation in any detail (see point
10.4).

2.3 The next comment about 100x143 and 100x217 TT is strange. These
spectra are much noisier that the 143x143, 143x217, 217x217 spectra at
high multipoles (ell > 1000), so they add nothing. At low multipoles
(ell < 500) we are signal dominated and have a high level of
consistency between the spectra, so again the 100x143 and 100x217
spectra add nothing -- and to use them we would have to use more
foreground parameters. It was the decision of one of us (GE) not to
use these spectra in the 2013 and subsequent Planck likelihood and
params papers; no referee of those papers has questioned this point.


The referee says several times that 100 GHz is less affected by dust,
 which is true.  But we show in Sect. 7.4, and discuss in detail, that
 dust cleaned 143 GHz is `cleaner' than dust cleaned 100 GHz. The
 additional contaminants at 100 GHz is primarily CO emission + a bit
 of synchrotron.  Dust cleaned 143 is cleaner than 100 GHz at ell <
 500. Dust cleaned 143 and 217 are MUCH cleaner than 100 GHz at higher
 multipoles, because 545 template cleaning removes most of the CIB and
 unresolved point sources at 143 GHz and 217 GHz, but does not remove
 the radio point source contribution at 100 GHz (or at 143 GHz) . Thus
 we use only 143x143, 143x217 and 217x217 in our cleaned
 likelihood. All of this is explained in great detail in the paper.

3.1 The weights $w_i$ are defined at the end of page 4, and $\Omega_i$
is defined after Eq. 2.2. We use the PLA masks in TT which are
described in the Planck papers and described in the PLA.


3.2 The referee says that it isn't clear which mask is used for which
likelihood.  This is strange because Table 11 lists the masks used for
each likelihood. You can see from this Table that we tested
polarization spectra on a range of masks from 60-80\% of sky -- and
this is illustrated graphically in Fig. 12.6. We did not, as the
referee says, limit the sky fraction to 50 or 60\% of sky. We discuss
point source masking in polarization. It is only important to remove a
few bright polarized sources, but we decided on overkill and applied
the 143 GHz point source mask.

We could give the sky fractions in the caption to Fig. 3.2, though the
names of the masks do tell the reader the sky fractions.


4.1 The SWB are polarized, but are not used to construct polarization
maps. The maps are exactly as in the PLA. The decision on whether to
make deset maps publically available was taken by the Planck Science
Team, not by us. We were given permission to use the detset maps in
this paper by the Planck Science Team. It is perfectly clear from the
footnote that the detset maps are not in the PLA. As we say in the
paper, the 2018 detset maps are nearly identical to the 2015 detset
maps which are available on the PLA. The only differences is that the
2015 maps have slightly lower noise because rings at end of the
mission were included in 2015 but excluded in 2018. Had we used the
2015 detset maps in this paper, the differences would have been
imperceptible. (We know this because we replaced all of the
figures/numbers using 2015 detset maps in an earlier draft with
results for the 2018 detset maps.)


4.2 We are correct -- it is `lower multipole cuts'. (We reject the
data at lower multipoles).

5.1 Why criticise us for the Planck products? These maps are what have
been delivered to the PLA. The holes are actually defined by the
condition number of the polarization solution. We can clarify what is
meant by odd-even pointing rings -- the scanning rings are assigned
numbers, 1, 2, 3.... so one can make maps with odd rings or even
rings.

Noise estimation is a major problem for Planck. The purpose of
Fig. 5.1 is to show that it is difficult to get reliable noise
estimates at better than the 2-3\% level (if that). The autospectra
will contain correlated noise and so provide only a rough guide. The
HRD spectra underestimate the noise at low multipoles (even the FFP8,
FFP10 simulations show this) and the OED overestimate the noise at low
multipoles. The latter is unimportant for TT, which is signal
dominated over most of the multipole range) but has an effect on EE
which is noise dominated over most of the multipole range.

It is surely obvious that since EE carries very little weight on the
TTTEEE likelihood that the relatively small underestimates of chi**2
in EE have very little impact on cosmological parameters or their
posterior widths. There will be an impact on parameters from the EE
block alone, but these are really used only for consistency tests.


5.2 The correlated noise comes primarily from 4K line removal, which
is not modelled in the E2E Planck simulations (see point 10.4).  You
cannot use the Planck simulations to correct for correlated noise. We
don't use the fits in Fig 5.2 to very high multipoles where the OED
spectra become noisy, and we consider the detset likelihood to be less
reliable than the HM likelihoods because of correlated noise. But you
can see comparisons of the spectra in Figs. 11.2, 11.7 and 12.5, and
you can also see that the parameters from the detset likelihood (for
base LCDM) are in very good agreement with those of the HM likelihood.

 Concerning Fig. 6.1, of course correcting for correlated noise will
 increase the noise levels in these plots at high multipoles. But this
 is not the point -- the key point is that small effective calibration
 corrections eliminate almost all of the scatter at multipoles < 1000
 (the correlated noise corrections also reduce the scatter at ell <
 1000, but this is a much smaller effect). These tests gives
 incredible support that each detector is seeing the SAME SIGNAL on
 the sky at multipoles < 1000.


6.1 Agree that thermal fluctuations can contribute to non white noise.
Eq. (6.3a) and (6.3b) are what we use. Eqs. (6.4-6.5) are based on an
approximation developed by Hivon, which as far as we know, has not
been published in a refereed paper.

6.2 I really don't understand what the referee is concerned about
here. We state very clearly that the beam modelling will produce a
small transfer function variation at low multipoles, but for spectra
at say $\ell > 100$ this transfer function should become an effective
calibration factor which we then go on to determine. The calibration
factors come out to be very close to unity. This is very good
news. The main beam eigenmodes are tiny, they are so small that since
2015 we do not propagate main beam errors into the cosmological
analysis. There is no possibility of beam transfer function
errors affecting parameters such as n_s. Also, look at the remarkable
consistency of the inter-frequency residuals as plotted in
Fig. 13.11. There is no hint of a transfer function across these
frequencies, which have very different beams.

6.3 NO! The calibrations are relative to a TT best fit theoretical
model. You can argue that we have to assume a model, which is a strong
assumption, but given this assumption, our results are consistent with
MAP based polarization efficiencies as given in Table 6.  We make the
case that the Plik team biased their polarization likelihood by using
EE coefficients which are noiser and less reliable than the TE
coefficients.  This difference (as acknowledged in the revised Planck
Params paper) is responsible for the Plik TTTEEE results on A_L and
Omega_k which do not agree with ours. Plik have used TE coefficients
and reproduce results close to ours.  This should end this debate. We
can explicitly quote from the revised Planck Params paper to make this
clearer.


6.4 Yes, in the top two plots in Fig 6.3, the beam model is lower than
the triplets. You have to remember however that the TP leakage
correction is itself small. The primary systematic is polarization
efficiency. It doesn't make very much difference whether we used the
dotted or solid lines for cosmological parameters.


7.  We say very clearly that dust emission is remarkably universal
over most of the sky (i.e. a dust template rescaled with a single
template coefficient describes dust emission over most of the
sky). That is what we mean by universality -- we could try and
rephrase this, eg.  universality means no angular variations in the
spectral index.

7.1 Getting reliable errors for the numbers in Table 7 is very
difficult. We have not done so because we template clean in the
spectral domain, the minimum of Equ. 7.8 is very broad. As explained
on page 39, the residuals of the cleaned spectra vary as the square of
the error in the cleaning coefficients. So, as far as spectra cleaning
is concerned the results are insensitive to the exact values of the
cleaning coefficients. Had we calculated errors, they would not have
been used in making cleaned spectra. The quantities $\alpha^T_m$, $c$
and $c^\prime$ are DEFINED by Eqs. (7.1a) and (7.1b).

I don't understand the comments about the effects of point source
masks on the dust power spectra.  This is discussed in detail in
Section 7.2, which includes Fig 7.2. Our use of mask differenced power
spectra takes out extragalactic components so you can really see what
is happening with dust. This has not been done in any other paper that
I have seen.


7.2 Yes, we could repeat Eq. 5.4 in Sect. 7. I am not really concerned
about high galactic cirrus.  What I am concerned about is the dust
contributions on the masks used in cosmological analysis. Fig. 7.1 is
an amazing figure and shows that the dust is under control over the
frequency range 217-857 GHz.  The scatter in the pink points at
multipoles < 1500 is dominated by CMB/foreground cross-correlations.
This dominates over instrument noise at 217 GHz. One can also see this
beautifully from Fig. 7.4.


7.3 I have explained the lack of errors already. We could add a few
more words about dust cleaning. Table 7.1 shows that for low amplitude
foregrounds, the CMB distorts the map based coefficients (Eq. (7.1) )
this is why we subtract the SMICA map (Eq. 7.1b) which gives results
closer to the spectrum based cleaning. The differences between columns
4 and 5 are quite small, but I haven't investigated the precise reason
for the differences.


7.4.  I really don't know what you want us to say here. Template
cleaning fails close to the galactic plane. All component separation
methods fail close to the galactic plane -- you can see this in any of
the Planck Foreground cleaning papers. The 100 GHz spectrum at low
multipoles is compared to the higher frequency spectra in Fig 9.1.
You can see that the residuals for 100x100-143x143 GHz are small and
that leaves very little room for synchrotron.  The main contribution
to these residuals is from CO emission not synchrotron. This is not
explored in this paper because the residuals in Fig 9.1 are already so
small that they have no impact whatsoever on cosmology.  Remember that
the first CMB peak at ell \sim 200 has an amplitude of about 6000
muK^2.

 We cover the point about more frequencies in the paper. If the
 foregrounds are more complex at low frequencies, then you gain very
 little by extending the frequency range, and can actually make things
 significantly worse (as in early versions of commander). We stay at
 the high frequencies because dust appears to be universal at high
 frequencies.

 It is remarkable that we can have such a different reaction to Fig
 7.9.  As you increase sky coverage, the cosmic variance will change,
 so points will move about a bit. However, the spectra look almost the
 same, and if you look across frequencies, they behave in the same way
 i.e. independent of frequency. This is very, very strong evidence of
 the effectiveness of template cleaning (and therefore of
 universality). The dispersion is within a few muK^2, i.e within
 0.08\% of the cosmogical signal -- and as a referee your reaction is
 `so what?'. This is an astonishing reaction.

The easiest way to see the effectiveness of 545 cleaning is to look at
Fig 11.4. 545 cleaning removes most of the clustered CIB and
unresolved dusty point sources. It leaves very little residual
foreground at high multipoles in the 143x217 and 217x217 spectra.


8.  We have done many, many tests of foregrounds in polarization. We
have seen no evidence of polarized synchrotron at 100 or 143 GHz. We
show all the cleaned polarization spectra in Figs. 8.3, 8.4, and
8.5. There is no excess after dust cleaning that would have any impact
on cosmology.

    You can easily see from Eq. 7.12 that the minima are broad and as
    with Table 7 we don't quote errors on the cleaning
    coefficients. But the E and B coefficients give you an idea of the
    errors. We could put polarization coefficients on Fig. 7.6, but
    these would only cover the frequency range 100-353 GHz. The SED in
    polarization is consistent with the SED in temperature.

 You are correct, Sect. 7.2 gives alpha = 0.69 for TT (not 0.67).


8.1 I don't understand the comment. When we use half mission maps we
do not use cotemporal spectra. For 143x217, we have 143HM2x217HM1 and
143HM1x217HM2, but for 143x143 we have only 143HM1x143HM2.



  Excess in 217 Q/U maps is caused by systematic errors.  We can add
  more references to the SROLL paper which says the same thing with a
  lot of supporting evidence. This is why the Planck tau constraint is
  based exclusively of 100x143 EE spectra.

 We show each polarization spectrum with and without cleaning compared
 to the best fit TT model. In every case, the cleaning brings the
 spectra into agreement with the expectations of the TT model. I
 simply cannot undestand why, faced with this you would say `this is
 not demonstrated in this paper. Please clarify or remove'. What more
 could we do?

In TE/ET the dust corrections CAN HAVE EITHER SIGN, i.e. the TE/ET
spectra can go up or down after cleaning. This is clearly demonstrated
in the plots. Yet Plik correct dust emission in TE by fitting power
law dust templates. This is clearly wrong.



9.1 Page 53 `This reduces degeneracies with other foreground
components....'. We have tested this and that is what happens. If one
allows a lot of freedom in the calibrations, the dust amplitudes will
shift as will other foreground parameters. It is surely self evident
that if we can fix the relative calibrations accurately, as we have
done here, then the foreground model will have less freedom. That is
all we are saying.


9.1.3 The analysis of absolute calibration is, we agree, not
satisfactory. The point here is that we need to know the variance on
the effective calibration at ell \sim 1000. The absolute calibration
of Planck as measured by the Solar dipole is discussed in the HFI DPC
paper, and is much better than the 0.25\% adopted here. We had to pick
a representative number -- 0.1\% in the spectrum domain based on
Fig. 6.1 might have been a more justifiable choice. In the end we
decided to stay consistent with the Planck papers which used 0.25\% on
y_cal.

9.3.3 The spectrum from the Planck tSZ paper is well fitted by the
Efstathiou and Migliaccio (EM) model. We use the EM model with a free
amplitude (as in the Planck parameter papers) which we determine by
fitting the spectra. The resulting amplitude is more reliable than the
amplitude derived in the tSZ paper.

The nuisance parameters are listed in Table 10, together with the
prior ranges. I couldn't find any reference to `12' nuisance
parameters. The six parameters in the cleaned likelihod are discussed
in Sect. 9.4.


10.1 The Planck team did not specifically produce a mask for strong
polarized sources (though it should have done).  We have experimented
with such masks, but as we have said, in the end we decided to be
conservative and adopted the 143 GHz point source mask in
polarization.


In full mission, one is using almost all of the data in TT and EE, so
the noise is lower than in the half-mission TT and EE spectra.

I don't want to add columns to Table 11. All of the polarization
spectra are cleaned with 353 for all likelihoods.  TT cleaning uses
545 GHz. This is discussed extensively in the text.

10.3 The comment is pedantry. The constraint on tau from TT alone is
very weak. Nobody would think it sensible to run a likelihood using
only TT at ell> 30.


10.4 The referee comments in several places that we have not used E2E
simulations. We have used such simulations but they are simply not
accurate enough. We have worked extensively with these
simulations. The main drawbacks are: (a) mismatch of the noise
compared to the actual noise at the tod and map level; (b) major
mismatches of foregrounds compared to the real world; (c) absence of
many systematics such as 4k line removal, thermal fluctuations,
deglitching, beam efficiencies etc etc. We have had to develop
techniques to test many of these things using the data, as described
in this paper.

The choice of lmin = 30 is not critical and follows the choice made in
the Planck papers.

11.1 Fig 11.2 -- the differences between these spectra are shown in
Fig 11.3 which gives dispersions and has accurate errors on the
differences. This is the plot that you should be looking at if you
want to assess the consistency of the spectra.

11.2 Why would you expect the impact of 545 cleaning to be striking in
Fig 11.3? The standard foreground model works really well because of the
limited sky coverage. So what you see is smaller residuals at
multipoles ell \simlt 1000 in the cleaned spectra because
CMB/foreground cross correlations are surpressed. However, it is this
suppression of CMB/foreground cross-correlations that allows us to
extend sky coverage at 143 and 217 to produce Fig. 13.11. The standard
foreground modelling fails catastrophically in this case.


11.4 Although the noise can be reduced using the full mission
likelihood, one pays a price because of correlated noise. So we have
used it as a consistency check here. The wording in the paper is
precise.  The correlated noise in the detsets is very likely a failure
in the data processing, related to 4K line removal. We are currently
analysing the new `NPIPE' maps which show very little correlated noise
at high multipoles.


12.1 As explained above the chi^2 for EE spectra involving 100 GHz are
low (though not hugely low) but EE contributes very little to the
TTTEEE likelihood. The TT/TE chi^2 are acceptable. These reduced chi^2
values are actually much closer to unity that those of the Plik 2018
likelihood quoted in the 2018 Planck Likelihood and Params papers!



12.2 We have many TE/ET and EE spectra in the detsets (72 TE/ET
spectra). We have only two 353 detsets, so we can't clean these
spectra with 353 GHz without picking up correlated noise.


12.5  Fig 12.5 looks OK to me at high multipoles. 


13.6 If you restrict the spectra at ell> 1000, the dust amplitude is
indeed subdominant. However, if you allow the amplitude to vary, it
will be degenerate with other forerounds and so will explore
unphysical values. You can try to damp this down by putting a prior on
the dust amplitude, then the dust amplitude will just sample the prior
with impact on the other foreground parameters. At low multipoles, the
dust is dominant and you can pin its amplitude accurately. However, if
you clean the spectra, there is no dust (and very little CIB) to worry
about, so you become insensitive to foreground modelling.  There is
negligible correlation between low and high multipoles in the
spectra. The analysis presented here uses a more powerful likelihood
and is more robust than the analysis in [100] because of the independence
of the multipole ranges and insensitivity to foregrounds. The analysis in
[100] uses the `plik light' code which samples the foreground solutions
from the full multipole range of the likelihood. 

14.1 `illustrates the extreme sensitivity of A_L to the nuisance
parameters'. This is poorly worded, it is meant to refer to the
difference between 12.5HMcl TT and 12.1HM TT not between 12.1HM TT and
the 2018 Camspec likelihood.

14.4 Yes B-mode constraints are now dominating and the main
contribution of Planck is to constrain n_s.


15 Conclusions

   The 12.5HM cleaned likelihood is publically available and is being
   used by others. The foreground templates are avaliable from the
   PLA, since they are part of the 2018 Plik and CamSpec
   likelihoods. Almost all of the data used in this paper are
   publically avaliable, including masks. The polarization specific
   masks used in this paper are not available but they can easily be
   constructed from the 353GHz polarization maps if required. The avialability of
   code and data from ground based experiments is patchy. Maps, codes and supplementary
   products are not made public by the SPT collaboration.







==> referee_reply2.tex <==

We have waited two months to receive a one page report, apparently by
the same referee. As we stated in our response to the first referee
report, we disagreed with many of the referee's technical criticisms
of our analysis. There was also a lack of appreciation: (a) that the
paper broke new ground by increasing the sky coverage used in the
temperature and polarization likelihood, substantially strengthening
the case for the base LCDM cosmology; (b) this type of analysis cannot
be summarized in a few pages because the details matter.  As stated in
our earlier response, we are therefore not prepared to make major
changes to the paper.

We specifically asked that the paper be sent to another referee since
it was unlikely that we could achieve a compromise with the first
referee.  It is disappointing that this apparently hasn't been done. 
We therefore ask that the Editor make a decision on this paper. If JCAP 
are not interested in this paper, then we will update astroph to the latest
version submitted to you, and either submit to another journal or
leave it on astroph as an unrefereed paper.  Removing important
details merely to shorten the paper would suppress information flow
and we are not prepared to do that.  It would be far more preferable
to us to have the full paper avaliable on astroph.


                George Efstathiou
                Steven Gratton

